Wave Propagation of Visual Stimuli in Focus of Attention

Fast reactions to changes in the surrounding visual environment require efficient attention mechanisms to reallocate computational resources to most relevant locations in the visual field. While current computational models keep improving their predictive ability thanks to the increasing availability of data, they still struggle approximating the effectiveness and efficiency exhibited by foveated animals. In this paper, we present a biologically-plausible computational model of focus of attention that exhibits spatiotemporal locality and that is very well-suited for parallel and distributed implementations. Attention emerges as a wave propagation process originated by visual stimuli corresponding to details and motion information. The resulting field obeys the principle of "inhibition of return" so as not to get stuck in potential holes. An accurate experimentation of the model shows that it achieves top level performance in scanpath prediction tasks. This can easily be understood at the light of a theoretical result that we establish in the paper, where we prove that as the velocity of wave propagation goes to infinity, the proposed model reduces to recently proposed state of the art gravitational models of focus of attention.

==> Makefile <==
main = neurips_foa_2020

default: draft paper 
paper: $(main).pdf
draft: $(main).draft.pdf

maininc = exp.tex introduction.tex poisson.tex reg.tex supp.tex 
sources = $(main).tex $(maininc)
sourcesdraft = $(main).draft.tex $(maininc)

$(main).pdf: $(sources)

$(main).draft.pdf: $(sourcesdraft)



%.pdf: %.tex
	pdflatex $*
	@while ( grep "Rerun to get cross-references" $*.log >/dev/null ); do \
	echo '** Re-running LaTeX **';  \
		pdflatex $*;          \
	done
	@if (grep "LaTeX Warning: There were undefined references." $*.log >/dev/null); then \
	echo '** Running Biber **'; \
		biber $*; \
	fi
	@while ( grep "LaTeX Warning: There were undefined references." $*.log >/dev/null ); do \
	echo '** Re-running LaTeX **';  \
		pdflatex $*;          \
	done

%.draft.tex: %.tex
	sed -e "s/%%DRAFT%%//" $< >$@
	echo '%WARNING: File automatically generated by make DO NOT edit!' | cat - $@ > temp && mv temp $@

clean:
	rm *.aux *.log *.bbl *.blg *.pdf *.bcf *.out *.xml *.draft.tex *.gz



==> figures.tex <==
\begin{figure}[htb]
    \centering 
\begin{subfigure}{0.33\textwidth}
  \includegraphics[width=\linewidth]{Images_for_submission/1D}
\end{subfigure}\hfil 
\begin{subfigure}{0.33\textwidth}
  \includegraphics[width=\linewidth]{Images_for_submission/2D}
\end{subfigure}\hfil 
\begin{subfigure}{0.33\textwidth}
  \includegraphics[width=\linewidth]{Images_for_submission/3D}
\end{subfigure}

\vspace{1pt}

\begin{subfigure}{0.33\textwidth}
  \includegraphics[width=\linewidth]{Images_for_submission/1DW}
\end{subfigure}\hfil 
\begin{subfigure}{0.33\textwidth}
  \includegraphics[width=\linewidth]{Images_for_submission/2DW}
\end{subfigure}\hfil 
\begin{subfigure}{0.33\textwidth}
  \includegraphics[width=\linewidth]{Images_for_submission/3DW}
\end{subfigure}

\vspace{5pt}

\begin{subfigure}{0.33\textwidth}
  \includegraphics[width=\linewidth]{Images_for_submission/4D}
\end{subfigure}\hfil 
\begin{subfigure}{0.33\textwidth}
  \includegraphics[width=\linewidth]{Images_for_submission/5D}
\end{subfigure}\hfil 
\begin{subfigure}{0.33\textwidth}
  \includegraphics[width=\linewidth]{Images_for_submission/6D}
\end{subfigure}

\vspace{1pt}
\begin{subfigure}{0.33\textwidth}
  \includegraphics[width=\linewidth]{Images_for_submission/4DW}
\end{subfigure}\hfil 
\begin{subfigure}{0.33\textwidth}
  \includegraphics[width=\linewidth]{Images_for_submission/5DW}
\end{subfigure}\hfil 
\begin{subfigure}{0.33\textwidth}
  \includegraphics[width=\linewidth]{Images_for_submission/6DW}
\end{subfigure}

\caption{Fixations for the $\h$ model (top) and $\dw$ model (bottom) obtained
in five seconds of exploration.
Images from the CAT2000 training set.}
\label{fig:images}
\end{figure}



\begin{figure}[htb]
    \centering 
\begin{subfigure}{0.45\textwidth}
  \includegraphics[width=\linewidth]{Images_for_submission/VID_D_0}
\end{subfigure}\hfil 
\begin{subfigure}{0.45\textwidth}
  \includegraphics[width=\linewidth]{Images_for_submission/VID_DW_0}
\end{subfigure}

\vspace{1pt}

\begin{subfigure}{0.45\textwidth}
  \includegraphics[width=\linewidth]{Images_for_submission/VID_D_1}
\end{subfigure}\hfil 
\begin{subfigure}{0.45\textwidth}
  \includegraphics[width=\linewidth]{Images_for_submission/VID_DW_1}
\end{subfigure}

\vspace{1pt}
\begin{subfigure}{0.45\textwidth}
  \includegraphics[width=\linewidth]{Images_for_submission/VID_D_2}
\end{subfigure}\hfil 
\begin{subfigure}{0.45\textwidth}
  \includegraphics[width=\linewidth]{Images_for_submission/VID_DW_2}
\end{subfigure}

\vspace{1pt}
\begin{subfigure}{0.45\textwidth}
  \includegraphics[width=\linewidth]{Images_for_submission/VID_D_3}
\end{subfigure}\hfil 
\begin{subfigure}{0.45\textwidth}
  \includegraphics[width=\linewidth]{Images_for_submission/VID_DW_3}
\end{subfigure}

\vspace{1pt}
\begin{subfigure}{0.45\textwidth}
  \includegraphics[width=\linewidth]{Images_for_submission/VID_D_4}
\end{subfigure}\hfil 
\begin{subfigure}{0.45\textwidth}
  \includegraphics[width=\linewidth]{Images_for_submission/VID_DW_4}
\end{subfigure}

\vspace{1pt}
\begin{subfigure}{0.45\textwidth}
  \includegraphics[width=\linewidth]{Images_for_submission/VID_D_5}
\end{subfigure}\hfil 
\begin{subfigure}{0.45\textwidth}
  \includegraphics[width=\linewidth]{Images_for_submission/VID_DW_5}
\end{subfigure}

\caption{Dynamical evolution of the potential in the $\h$ model (left) and
$\dw$ model (right) in the case of
a $5$ seconds example video. }
\label{fig:videos}
\end{figure}

==> old_calc/calc.tex <==
\section{Backup}
The generic term in the expansion~\eqref{expansion} forces us to consider
the following integral:
\[
\frac{1}{c^n}\int_{|z|}^{ct}\frac{\tau^n}{(\tau^2-|z|^2)^{1/2}}\, d\tau
=
\frac{1}{2}\frac{|z|^n}{c^n}\left(\sqrt{\pi}\frac{\Gamma(-n/2)}{\Gamma((1-n)/2)}
-\Beta(|z|^2/(ct)^2;-n/2,1/2)\right)
\]
or
\[
\begin{aligned}
\frac{1}{c^n}\int_{|z|}^{ct}\frac{\tau^n}{(\tau^2-|z|^2)^{1/2}}\, d\tau
&=
\frac{1}{2}\frac{|z|^n}{c^n}\left(\Beta(-n/2,1/2)
-\Beta(|z|^2/(ct)^2;-n/2,1/2)\right)\\
&=
\frac{1}{2}\frac{|z|^n}{c^n}\Beta(-n/2,1/2)\left(1
-I(|z|^2/(ct)^2;-n/2,1/2)\right)\end{aligned}
\]
Notice that when $|z|=ct$, then
$\Beta(1,-n/2,1/2)=\Beta(-n/2,1/2)=\sqrt{\pi}\Gamma(-n/2)/\Gamma((1-n)/2)$ so
that the above expression is identically null, coherently with the
fact that we are integrating on a null interval.

\medskip
\centerline{*\quad*\quad*}
\medskip

\meno
{\bf Wave equation (1D).} Let us study the problem in $1-D$.
In this case the solution to Eq.~\eqref{c-wave} is
\[u(x,t)=\frac{1}{2}\bigl(f(x-ct)+f(x+ct)\bigr)
+\frac{1}{2c}\int_{x-ct}^{x+ct}g(y)\, dy,\]
then
\[w_s(x,t)=\frac{c}{2}\int_{x-ct}^{x+ct}\mu(y,s)\, dy,\]
hence
\[\varphi(x,t)=\frac{c}{2}\int_0^t\int_{x-c(t-s)}^{x+c(t-s)}\mu(y,s)\, dyds.\]
Performing the usual change of variables $c(t-s)=\tau$ we finally get
\[\varphi(x,t)=\frac{1}{2}\int_0^{ct}\int_{x-\tau}^{x+\tau}\mu(y,t-\tau/c)\,
dyd\tau.\]
Setting $z=y-x$ we get
\[
\varphi(x,t)=\frac{1}{2}\int_0^{ct}\biggl(\int_{-\tau}^{\tau}\mu(x+z,t-\tau/c)\,
dz\biggr)\,d\tau=
\frac{1}{2}\int_{-ct}^{ct}\biggl(\int_{|z|}^{ct}\mu(x+z,t-\tau/c)\,
d\tau\biggr)dz.
\]
